Yi: Open Foundation Models by 01.AI

We introduce the Yi model family, a series of language and multimodal models that demonstrate strong multi-dimensional capabilities. The Yi model family is based on 6B and 34B pretrained language models, then we extend them to chat models, 200K long context models, depth-upscaled models, and vision-language models. Our base models achieve strong performance on a wide range of benchmarks like MMLU, and our finetuned chat models deliver strong human preference rate on major evaluation platforms like AlpacaEval and Chatbot Arena. Building upon our scalable super-computing infrastructure and the classical transformer architecture, we attribute the performance of Yi models primarily to its data quality resulting from our data-engineering efforts. For pretraining, we construct 3.1 trillion tokens of English and Chinese corpora using a cascaded data deduplication and quality filtering pipeline. For finetuning, we polish a small scale (less than 10K) instruction dataset over multiple iterations such that every single instance has been verified directly by our machine learning engineers. For vision-language, we combine the chat language model with a vision transformer encoder and train the model to align visual representations to the semantic space of the language model. We further extend the context length to 200K through lightweight continual pretraining and demonstrate strong needle-in-a-haystack retrieval performance. We show that extending the depth of the pretrained checkpoint through continual pretraining further improves performance. We believe that given our current results, continuing to scale up model parameters using thoroughly optimized data will lead to even stronger frontier models.

==> 060_in_depth_study.tex <==
% \subsection{Training Dynamics}

\subsection{In-Context learning}
\input{images/fig_icl}

\subsection{SFT Data Quality}

==> app_more_exp.tex <==
\input{tables/tab_commonsense}
\input{tables/tab_mmlu}
\input{tables/tab_qa}
% \input{tables/tab_long_context}

==> tables/tab_code.tex <==
\begin{table}
  \centering
  \begin{tabular}{lcccc}
    \toprule
    & \multirow{2}{*}{\bf Size} & \multirow{2}{*}{\bf Avg} & \multicolumn{1}{c}{\bf Human-Eval} & \multicolumn{1}{c}{\bf MBPP} \\
    & & & pass@1 & pass@1 \\
    \midrule
    \bf GPT-3.5 & - & 54.8 & 48.1 & 61.4 \\
    \bf GPT-4 & - & \textbf{65.3} & \textbf{67.0} & \textbf{63.6} \\
    \gmidrule
    % \midrule
    \bf Falcon & 180B & 23.8 & 0.61 & 47.0 \\
    \gmidrule
    \multirow{2}{*}{\bf Qwen} & 7B & 32.0 & 29.9 & 34.0 \\
     & 14B & 40.6 & 32.3 & 48.9 \\
    \gmidrule
    \multirow{2}{*}{\bf Baichuan 2} & 7B & 23.3 & 18.3 & 28.3 \\ 
    & 13B & 23.4 & 20.7 & 26.1 \\
    \gmidrule
    \multirow{3}{*}{\bf L\textsmaller{LaMA} 2} 
    & 7B & 13.8 & 12.8 & 14.8 \\
    & 34B & 27.8 & 22.6 & 33.0 \\
     & 70B & 38.4 & 31.7 & 45.0 \\
     \gmidrule
    \bf Mistral & 7B & 39.0 & 30.5 & 47.5 \\
    \gmidrule
    \bf InternLM & 20B & 34.8 & 28.1 & 41.4 \\
    \gmidrule
    \bf Skywork & 7B & 18.1 & 13.4 & 22.8 \\
    % \midrule
    \gmidrule
    \multirow{2}{*}{\bf Yi} & 6B & 21.1 & 15.9 & 26.3 \\
     & 34B & 32.1 & 23.2 & 41.0 \\
    \bottomrule
  \end{tabular}
  \caption{Code generation results on Human-Eval and MBPP.
  % \qj{pass@1 or pass@80?}. 
  We report 0-shot with greedy decoding results for pass@1 scores.
  % \alex{what kind of prompt did we use? do we test the numbers of all these models on our own, or we copy the number from their papers?}
  }
  \label{tab:code}
\end{table}

==> tables/tab_commonsense.tex <==

\begin{table}[t!]
  \centering
  \resizebox{.99\columnwidth}{!}{
  \begin{tabular}{@{}lcccccccccccc@{}}
\toprule
              &  \bf Size  & \bf Avg & \bf  BoolQ  &  \bf PIQA & \bf SIQA  & \bf  HellaSwag & \bf WinoGrande & \bf  ARC-e & \bf  ARC-c & \bf  OBQA \\
\midrule
% \midrule
\bf GPT-3.5 & - & 83.1 &   87.2 & 81.7 & 72.4 & 79.5 & 81.6 & 88.9 & 83.7 & 89.6 \\
\bf GPT-4 & - & \textbf{89.3} &  \textbf{90.6} & \textbf{89.2} & 70.1 & \textbf{91.4} & \textbf{87.5} & \textbf{95.4} & \textbf{93.6} & \textbf{96.6} \\
\gmidrule
\multirow{2}{*}{\bf PaLM} & 62B & - &  84.8 & 80.5 & - & 79.7 & 77.0 & 75.2 & 52.5 & 50.4 \\ 
& 540B & - & 88.0 & 82.3 & - & 83.4 & 81.1 & 76.6 & 53.0 & 53.4 \\
 
 % \midrule
 \gmidrule
\bf Falcon & 180B & 74.4 & 86.8 & 85.0 & 65.9 & 85.9 & 80.1 & 82.2 & 60.8 & 48.8 \\
\gmidrule
\multirow{3}{*}{\bf L\textsmaller{LaMA} 2} 
 & 7B & 63.9 & 77.0 &  79.1 & 46.4 & 76.0 & 69.3 & 74.6 & 46.3 & 41.2 \\
  & 34B & 71.1 & 83.7 & 81.9 & 50.9 & 83.3 & 76.7 & 79.4 & 54.5 & 58.2 \\
   & 70B & 72.7 & 85.0 & 82.5 & 50.7 & 85.3 & 80.2 & 80.2 & 57.4 & 60.2 \\
\gmidrule
\multirow{2}{*}{\bf Qwen}
 & 7B & 63.9 & 67.8 & 78.2 & 68.2 & 76.9 & 68.5 & 72.0 & 46.4 & 94.8 \\
& 14B & 74.2 & 85.5 & 79.9 & 77.9 & 80.2 & 67.7 & 70.6 & 47.2 & 84.4 \\

 \gmidrule
\multirow{2}{*}{\bf Baichuan 2} & 7B & 62.4 & 63.2 & 77.4 & 51.1 & 72.2 & 68.5 & 72.9 & 42.0 & 52.2 \\
& 13B & 66.3 & 73.6 & 78.8 & 59.5 & 75.3 & 70.1 & 61.9 & 38.0 & 73.4 \\
 \gmidrule
\bf Mistral & 7B & 74.9 & 83.5 & 83.0 & 59.9 & 81.3 & 75.3 & 80.0 & 55.5 & 80.8 \\
\gmidrule
\bf InternLM & 20B & 78.3 & 87.5 & 80.3 & 72.8 & 78.1 & 69.4 & 86.1 & 81.7 & 87.6 \\
\gmidrule
\bf Skywork & 13B & 72.4 & 82.9 &  79.9    & 66.3     & 77.4      & 72.2 & 78.5 & 50.2 & 82.2 \\
% \midrule
% Open-L\textsmaller{LaMA} & 7B & 72.3 & 79.9 & 35.9 & 74.5 & 65.9 & 69.7 & 41.4 & 42.0 \\
% \midrule
% \multirow{2}{*}{L\textsmaller{LaMA}} & 7B & 75.5 & 79.2 & 37.2 & 76.2 & 69.9 & 72.8 & 44.7 & 41.4 \\
 \gmidrule
 \multirow{2}{*}{\bf Yi} 
 & 6B & 72.2 & 76.2 & 78.6 & 64.5 & 74.9 & 70.6 & 77.2 & 50.3 & 85.4 \\
 & 34B & 80.7 & 88.3 & 82.9 & \textbf{74.5} & 83.6 & 78.7 & 84.4 & 61.8 & 91.6 \\
  


\bottomrule

  \end{tabular}
  }
   \caption{Zero-shot Performance on Commonsense Reasoning Tasks. 
   % \alex{what kind of prompt did we use? do we test the numbers of all these models on our own, or we copy the number from their papers?}
   }
  \label{tab:commonsense_reasoning}
\end{table}

==> tables/tab_mmlu.tex <==
\begin{table}[t!]
  \centering
  \begin{tabular}{@{}lcccccc@{}}
\toprule
           &   \bf Size   & \bf Average  & \bf Humanity & \bf STEM  & \bf Social Science & \bf Other \\
\midrule
% \midrule
\bf GPT-4 & - & \textbf{86.40}   & \textbf{87.00} & \textbf{89.80}    & 75.70 & \textbf{83.60}    \\
\bf GPT-3.5 & - & 70.00 & 72.80 & 79.00    & 58.40 & 71.80   \\
\gmidrule
% \midrule
\bf Falcon  & 180B      & 70.38 & 66.88    & 59.16 & 80.79          & 76.76 \\
\gmidrule
\multirow{3}{*}{\bf  L\textsmaller{LaMA} 2} 
& 7B & 46.80 & 51.50 & 52.20 & 38.00 & 49.90 \\
& 34B & 62.60 & 59.40 & 52.10 & 71.80 & 69.20 \\
& 70B & 68.90 & 65.00 & 58.00 & 80.30 & 74.60 \\
\gmidrule
% L\textsmaller{LaMA} 33B hf     & 58.18 & 55.58    & 46.94 & 67.47          & 64.31 \\
\multirow{2}{*}{\bf Qwen}
 & 7B & 58.45 & 52.94    & 50.30 & 68.38         & 65.24 \\ 
 & 14B     & 66.69 & 61.57   & 59.59 & 76.24         & 72.19 \\
 \gmidrule
\multirow{2}{*}{\bf Baichuan 2} 
 &  7B & 54.70 & 60.30 & 62.10 & 45.10 & 56.40 \\
 & 13B     & 55.97 & 48.46    & 47.98 & 67.11          & 64.44 \\
 \gmidrule
\bf Mistral & 7B & 62.43 & 56.77 & 52.68 & 73.29 & 70.16 \\
\gmidrule
\bf InternLM & 20B & 62.10 & 67.4 & 70.6 & 51.8 & 63.8 \\
\gmidrule
\bf Skywork & 13B & 62.10 &  -    & -      & -      & - \\
% \midrule
\gmidrule
\multirow{2}{*}{\bf Yi} & 6B          & 63.24 & 59.10    & 53.15 & 73.83          & 69.26 \\
& 34B    & 76.32 & 73.17   & 68.03 & \textbf{85.11}          & 80.78 \\
\bottomrule

  \end{tabular}
   \caption{Detailed results of MMLU. 
   Yi-34B performs relatively well on humanity and social science, and we aim to improve the STEM performance  in future efforts. 
   }
  \label{tab:mmlu_table}
\end{table}


==> tables/tab_passkey.tex <==
\begin{table}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{lccccccccccccc}
    \toprule
    \multicolumn{2}{c}{Context Window} & \multicolumn{2}{c}{1K} & \multicolumn{2}{c}{4K} & \multicolumn{2}{c}{8K} & \multicolumn{2}{c}{16K} & \multicolumn{2}{c}{32K} & \multicolumn{2}{c}{64K}\\
    \midrule
    Model & Size & PG19 & PR & PG19 & PR & PG19 & PR & PG19 & PR & PG19 & PR & PG19 & PR\\
    \midrule
    Yi & 6B & 0.88 & 1.0 & 0.839 & 1.0 & 0.836 & 1.0 & 0.842 & 1.0 & 0.861& 1.0 & 0.981 & 0.0\\
    Yi & 34B & 0.788 & 1.0 & 0.745 & 1.0 & 0.736 & 1.0 & 0.734 & 1.0 & 0.869 & 1.0 & 1.357 & 0.945\\
    \bottomrule
    
      \end{tabular}
  }
   \caption{Yi with different context window in PG19 and Passkey Retrieval (PR) test. The PG19 are reported BPB with test set, and the EM score with 5 random digits passkey for the Passkey Retrieval.
   % \qj{EM score, remove the first column?}
   % \alex{Why the Yi6B model has 0 PR on 64K?}
   }
  \label{tab:context_window}
\end{table}

==> tables/tab_qa.tex <==
% \begin{table}
%   \centering
%   \begin{tabular}{lcccc}
% \toprule
% Model & Size & Avg & NaturalQuestions & TriviaQA \\
% \midrule
% GPT-3.5  & - & 45.4 & 27 & 63.8 \\
% GPT-4 & - & \textbf{57.7} & \textbf{40.4} & 75 \\
% \gmidrule
% Falcon & 180B & 59.5 & 31.7 & 87.3 \\
% \gmidrule
% \multirow{2}{*}{Qwen} & 7B & 39.6 & 14.6 & 64.5\\
% & 14B & - & 19.8 & - \\
% \gmidrule
% \multirow{2}{*}{Baichuan 2} 
% & 7B & 28.3 & 15.5 & 41.4 \\
% & 13B & 32.3 & 18.0 & 46.6 \\
% %\midrule
% %Open-L\textsmaller{LaMA} v2 & 7B & & & 11.4 & & & & 40 &  \\
% \gmidrule
% \multirow{3}{*}{L\textsmaller{LaMA} 2} & 7B & 48.9 & 25.7& 72.1  \\
%  & 34B & 58.7 & 32.8 & 84.5 \\
%  & 70B & 63.6 & \textbf{39.5} & \textbf{87.6} \\
% \gmidrule
% Mistral & 7B & 34.2 & 28.8 & 39.5 \\
% \gmidrule
% InternLM & 20B & 46.8 & 23.8 & 69.8 \\
% \gmidrule
% Skywork & 7B & - & - & 54.0 \\
% \gmidrule
% \multirow{2}{*}{Yi}
% & 6B & 40.8 & 16.7 & 64.9 \\
% & 34B & 54.6 & 27.7 & \textbf{81.5} \\
% \bottomrule

%   \end{tabular}
%    \caption{Comparison to open-source models on world knowledge understanding, (\textit{Left}) NaturalQuestions. Exact match performance. (\textit{Right}) TriviaQA. Zero-shot and few-shot
% exact match performance on the filtered dev set. For TriviaQA, we evaluate on Wiki validation subset.
% % \alex{what kind of prompt did we use? do we test the numbers of all these models on our own, or we copy the number from their papers?}
% }
%   \label{tab:world_knowledge}
% \end{table}


\begin{table}
  \centering
  \begin{tabular}{lcccccc}
    \toprule
    Model & Size & SQuAD & QUAC & BoolQ & NaturalQuestions & TriviaQA \\
    \midrule
    GPT-3.5 & - & - & - & 87.2 & 27 & 63.8 \\
    GPT-4 & - & - & - & 90.6 & \textbf{40.4} & 75.0 \\
    \gmidrule
    Falcon & 180B & 50.8 & - & 86.8 & 31.7 & 87.3 \\
    \gmidrule
    \multirow{2}{*}{Qwen} 
    & 7B & 74.1 & 36.7 & 67.8 & 14.6 & 64.5 \\
    & 14B & 84.2 & 47.8 & 85.5 & 19.8 & - \\
    \gmidrule
    Baichuan 2 & 13B & 74.0 & 39.7 & 73.6 & 18.0 & 46.6 \\
    \gmidrule
    \multirow{3}{*}{L\textsmaller{LaMA} 2} 
    & 7B & 67.2 & 39.4 & 77.4 & 25.7 & 72.1 \\
    & 34B & 78.8 & 44.3 & 83.7 & 32.8 & 84.5 \\
    & 70B & 82.6 & \textbf{49.4} & 85.0 & \textbf{39.5} & \textbf{87.6} \\
    \gmidrule
    Mistral & 7B & - & - & 83.5 & 28.8 & 39.5 \\
    \gmidrule
    InternLM & 20B & - & - & 87.5 & 23.8 & 69.8 \\
    \gmidrule
    Skywork & 7B & 70.9 & 41.0 & 82.9 & - & 54.0 \\
    \gmidrule
    \multirow{2}{*}{Yi}
    & 6B & 89.0 & 40.9 & 76.2 & 16.7 & 64.9 \\
    & 34B & \textbf{92.5} & 48.6 & \textbf{88.3} & 27.7 & \textbf{81.5} \\
    \bottomrule
  \end{tabular}
  \caption{Comparison of models on reading comprehension and world knowledge understanding.}
  \label{tab:qa}
\end{table}


==> tables/tab_reading_comprehension.tex <==

\begin{table}
  \centering
  \begin{tabular}{lccccc}
\toprule
Model & Size & Avg & SQUAD & QUAC & BoolQ\\
\midrule
GPT-3.5 & - & - & - & - & 87.2 \\
GPT-4 & - & - & - & - & 90.6 \\
\gmidrule
Falcon & 180B & - & 50.8 & - & 86.8 \\
\gmidrule
\multirow{2}{*}{Qwen} & 7B & 59.5 & 74.1 & 36.7 & 67.8\\
 & 14B & 72.5 & 84.2 & 47.8 & 85.5\\
 \gmidrule
Baichuan 2 & 13B & 62.4 & 74.0 & 39.7 & 73.6\\
% \midrule
% Open-L\textsmaller{LaMA} v2 & 7B & & & & & &  \\
\gmidrule
\multirow{3}{*}{L\textsmaller{LaMA} 2} & 7B & 61.3 & 67.2 & 39.4 & 77.4\\
& 34B & 68.9 & 78.8 & 44.3 & 83.7   \\
& 70B & 72.3 & 82.6 & \textbf{49.4} & 85.0 \\
\gmidrule
Mistral & 7B & - & - & - & 83.5\\
\gmidrule
InternLM & 20B & - & - & - & 87.5 \\
\gmidrule
Skywork & 7B & 64.9 & 70.9 & 41.0 & 82.9 \\
\gmidrule
\multirow{2}{*}{Yi}
& 6B & 68.7 & 89.0 & 40.9 & 76.2\\
& 34B & \textbf{76.5} & \textbf{92.5} & 48.6 & \textbf{88.3}\\
\bottomrule

  \end{tabular}
   \caption{Comparison to open-source models on reading comprehension, (SQUAD and QUAC).
   % \alex{what kind of prompt did we use? do we test the numbers of all these models on our own, or we copy the number from their papers?}
   }
  \label{tab:reading_comprehension}
\end{table}
